Three-dimensional Reconstruction of Coronal Plasma Properties from a Single Perspective

Much of our understanding of the state of coronal plasmas comes from observations that are optically thin. This means that light travels freely through the corona without being materially affected by it, which allows it to be easily seen through, but also results in a line-of-sight degeneracy which has previously thwarted attempts to recover the three-dimensional structure of the coronal plasma. However, although the corona is disorganized in the line-of-sight direction, it is highly organized in the field-aligned direction. This paper demonstrates how to exploit this organization to resolve the line-of-sight degeneracy in the plasma properties using a suitable magnetic field structure. A preliminary investigation with a potential field is shown, finding a solution which clearly resembles the real solar data, even with a single perspective. The results indicate that there is ample information in the resulting residuals that can be used to refine the magnetic field structure, allowing, for the first time, the optically thin plasma observations to speak directly to the magnetic field extrapolations.

==> aastex_journals.tex <==
%AASTEX journal commands
%Copied from version 5.2 (2005) by D. C. Jacobs 2008

\let\jnlatstyle=\rmfamily
\def\refatjnl#1{{\jnlatstyle#1}}%
\newcommand\aj{\refatjnl{AJ}}%
          % Astronomical Journal
\newcommand\actaa{\refatjnl{Acta Astron.}}%
  % Acta Astronomica
\newcommand\araa{\refatjnl{ARA\&A}}%
          % Annual Review of Astron and Astrophys
\newcommand\apj{\refatjnl{ApJ}}%
          % Astrophysical Journal
\newcommand\apjl{\refatjnl{ApJ}}%
          % Astrophysical Journal, Letters
\newcommand\apjs{\refatjnl{ApJS}}%
          % Astrophysical Journal, Supplement
\newcommand\ao{\refatjnl{Appl.~Opt.}}%
          % Applied Optics
\newcommand\apss{\refatjnl{Ap\&SS}}%
          % Astrophysics and Space Science
\newcommand\aap{\refatjnl{A\&A}}%
          % Astronomy and Astrophysics
\newcommand\aapr{\refatjnl{A\&A~Rev.}}%
          % Astronomy and Astrophysics Reviews
\newcommand\aaps{\refatjnl{A\&AS}}%
          % Astronomy and Astrophysics, Supplement
\newcommand\azh{\refatjnl{AZh}}%
          % Astronomicheskii Zhurnal
\newcommand\baas{\refatjnl{BAAS}}%
          % Bulletin of the AAS
\newcommand\caa{\refatjnl{Chinese Astron. Astrophys.}}%
  % Chinese Astronomy and Astrophysics
\newcommand\cjaa{\refatjnl{Chinese J. Astron. Astrophys.}}%
  % Chinese Journal of Astronomy and Astrophysics
\newcommand\icarus{\refatjnl{Icarus}}%
  % Icarus
\newcommand\jcap{\refatjnl{J. Cosmology Astropart. Phys.}}%
  % Journal of Cosmology and Astroparticle Physics
\newcommand\jrasc{\refatjnl{JRASC}}%
          % Journal of the RAS of Canada
\newcommand\memras{\refatjnl{MmRAS}}%
          % Memoirs of the RAS
\newcommand\mnras{\refatjnl{MNRAS}}%
          % Monthly Notices of the RAS
\newcommand\na{\refatjnl{New A}}%
  % New Astronomy
\newcommand\nar{\refatjnl{New A Rev.}}%
  % New Astronomy Review
\newcommand\pra{\refatjnl{Phys.~Rev.~A}}%
          % Physical Review A: General Physics
\newcommand\prb{\refatjnl{Phys.~Rev.~B}}%
          % Physical Review B: Solid State
\newcommand\prc{\refatjnl{Phys.~Rev.~C}}%
          % Physical Review C
\newcommand\prd{\refatjnl{Phys.~Rev.~D}}%
          % Physical Review D
\newcommand\pre{\refatjnl{Phys.~Rev.~E}}%
          % Physical Review E
\newcommand\prl{\refatjnl{Phys.~Rev.~Lett.}}%
          % Physical Review Letters
\newcommand\pasa{\refatjnl{PASA}}%
  % Publications of the Astron. Soc. of Australia
\newcommand\pasp{\refatjnl{PASP}}%
          % Publications of the ASP
\newcommand\pasj{\refatjnl{PASJ}}%
          % Publications of the ASJ
\newcommand\qjras{\refatjnl{QJRAS}}%
          % Quarterly Journal of the RAS
\newcommand\rmxaa{\refatjnl{Rev. Mexicana Astron. Astrofis.}}%
  % Revista Mexicana de Astronomia y Astrofisica
\newcommand\skytel{\refatjnl{S\&T}}%
          % Sky and Telescope
\newcommand\solphys{\refatjnl{Sol.~Phys.}}%
          % Solar Physics
\newcommand\sovast{\refatjnl{Soviet~Ast.}}%
          % Soviet Astronomy
\newcommand\ssr{\refatjnl{Space~Sci.~Rev.}}%
          % Space Science Reviews
\newcommand\zap{\refatjnl{ZAp}}%
          % Zeitschrift fuer Astrophysik
\newcommand\nat{\refatjnl{Nature}}%
          % Nature
\newcommand\iaucirc{\refatjnl{IAU~Circ.}}%
          % IAU Cirulars
\newcommand\aplett{\refatjnl{Astrophys.~Lett.}}%
          % Astrophysics Letters and Communications
\newcommand\apspr{\refatjnl{Astrophys.~Space~Phys.~Res.}}%
          % Astrophysics Space Physics Research
\newcommand\bain{\refatjnl{Bull.~Astron.~Inst.~Netherlands}}%
          % Bulletin Astronomical Institute of the Netherlands
\newcommand\fcp{\refatjnl{Fund.~Cosmic~Phys.}}%
          % Fundamental Cosmic Physics
\newcommand\gca{\refatjnl{Geochim.~Cosmochim.~Acta}}%
          % Geochimica Cosmochimica Acta
\newcommand\grl{\refatjnl{Geophys.~Res.~Lett.}}%
          % Geophysics Research Letters
\newcommand\jcp{\refatjnl{J.~Chem.~Phys.}}%
          % Journal of Chemical Physics
\newcommand\jgr{\refatjnl{J.~Geophys.~Res.}}%
          % Journal of Geophysical Research
\newcommand\jqsrt{\refatjnl{J.~Quant.~Spec.~Radiat.~Transf.}}%
          % Journal of Quantitiative Spectroscopy and Radiative Trasfer
\newcommand\memsai{\refatjnl{Mem.~Soc.~Astron.~Italiana}}%
          % Mem. Societa Astronomica Italiana
\newcommand\nphysa{\refatjnl{Nucl.~Phys.~A}}%
          % Nuclear Physics A
\newcommand\physrep{\refatjnl{Phys.~Rep.}}%
          % Physics Reports
\newcommand\physscr{\refatjnl{Phys.~Scr}}%
          % Physica Scripta
\newcommand\planss{\refatjnl{Planet.~Space~Sci.}}%
          % Planetary Space Science
\newcommand\procspie{\refatjnl{Proc.~SPIE}}%
          % Proceedings of the SPIE
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao

